Instance-Level Task Parameters: A Robust Multi-task Weighting Framework

Recent works have shown that deep neural networks benefit from multi-task learning by learning a shared representation across several related tasks. However, performance of such systems depend on relative weighting between various losses involved during training. Prior works on loss weighting schemes assume that instances are equally easy or hard for all tasks. In order to break this assumption, we let the training process dictate the optimal weighting of tasks for every instance in the dataset. More specifically, we equip every instance in the dataset with a set of learnable parameters (instance-level task parameters) where the cardinality is equal to the number of tasks learned by the model. These parameters model the weighting of each task for an instance. They are updated by gradient descent and do not require hand-crafted rules. We conduct extensive experiments on SURREAL and CityScapes datasets, for human shape and pose estimation, depth estimation and semantic segmentation tasks. In these tasks, our approach outperforms recent dynamic loss weighting approaches, e.g. reducing surface estimation errors by 8.97% on SURREAL. When applied to datasets where one or more tasks can have noisy annotations, the proposed method learns to prioritize learning from clean labels for a given task, e.g. reducing surface estimation errors by up to 60%. We also show that we can reliably detect corrupt labels for a given task as a by-product from learned instance-level task parameters.

==> sub_sections/sup_identifying_noise.tex <==
\section{Identifying Samples with Corrupt Labels}
For samples with corrupt labels for a task, instance-level task parameters attain a high value for that task.
In Section 4.6, we exploited this property to identify samples with noisy labels by simply sorting the instance-level 
task parameters and identifying the number of corrupt samples in the top 40\% of training dataset (when 
trained in the presence of 40\% label corruption). In Tables \ref{tab:hsm_noise_detection} 
and \ref{tab:cs_noise_detection} we 
report accuracies of identifying samples with corrupt labels (20\% and 40\% label corruption) for 
different tasks. Accuracies are evaluated by sorting instance-level task parameters in decreasing order 
of maginitude for the task that has corrupt labels, 
just before the first learning rate decay for model parameters, 20$^{th}$ epoch for models
trained on SURREAL and 60$^{th}$ epoch for models trained on CityScapes, 
see Sections \ref{sec:hsm_impl}, \ref{sec:cs_impl}. It is evident from the results that our
method is very effective in identifying samples with corrupt labels. 

% Noise identification results
\begin{table}[!t]
\captionsetup{font=small}
\noindent
\begin{adjustbox}{width=6.5cm}
\begin{tabular}{ccc} 
  \toprule 
  Corrupt Label & \% Corrupt & Detection Accuracy \\
  \midrule
  Pose \& Shape & 20\% & 97.79\% \\
   & 40\% & 98.99\% \\
  \midrule
  Segmentation & 20\% & 99.85\% \\
   & 40\% & 99.79\% \\
  \bottomrule
  \end{tabular}
\end{adjustbox}
{
  \caption{Percent of samples with corrupt labels found in top 20\% and top 40\% of SURREAL training dataset when sorted by magnitude of instance-level task parameters for 20\% and 40\% label corruption respectively.} \label{tab:hsm_noise_detection}
}
% \capbtabbox{
%   \begin{adjustbox}{width=6.0cm}
%   \begin{tabular}{ccc} 
%      \toprule 
%     Corrupt Label & \% Corrupt & Detection Accuracy \\
%     \midrule
%     Depth & 20\% & 100\% \\
%      & 40\% & 100\% \\
%     \midrule
%     Segmentation & 20\% & 97.14\% \\
%      & 40\% & 96.01\% \\
%     \bottomrule
%     \end{tabular}
%   \end{adjustbox}
%  }{
%   \caption{Percent of samples with corrupt labels found in top 20\% and top 40\% of CityScapes training dataset when sorted by magnitude of instance-level task parameters for 20\% and 40\% label corruption respectively.} \label{tab:cs_noise_detection}
% }
\end{table}

\begin{table}[!t]
\captionsetup{font=small}
\noindent
\begin{adjustbox}{width=6.5cm}
\begin{tabular}{ccc} 
     \toprule 
    Corrupt Label & \% Corrupt & Detection Accuracy \\
    \midrule
    Depth & 20\% & 100\% \\
     & 40\% & 100\% \\
    \midrule
    Segmentation & 20\% & 97.14\% \\
     & 40\% & 96.01\% \\
    \bottomrule
  \end{tabular}
\end{adjustbox}
{
  \caption{Percent of samples with corrupt labels found in top 20\% and top 40\% of CityScapes training dataset when sorted by magnitude of instance-level task parameters for 20\% and 40\% label corruption respectively.} \label{tab:cs_noise_detection}
}
\end{table}

==> sub_sections/sup_implementation_details.tex <==
\section{Implementation Details}

\subsection{Human Shape and Pose Estimation} \label{sec:hsm_impl}
We use the training and testing split prescribed by SURREAL~\cite{surreal2017} dataset. While the testing dataset is retained as is, the video sequences in training dataset are subsampled by taking every 50$^{th}$ frame, leading to a training dataset of size 99,341. Ground truth bounding boxes are inferred from ground truth segmentation masks. Ground truth bounding boxes are used to obtain a square crop of resolution $[256\times256]$, such that aspect ratio
of the human is maintained (see~\cite{varol2018bodynet} for more details). Multi-Task UNet architecture used in experiments is shown in Figure \ref{fig:hsm_arch}. The network and training code is implemented in PyTorch~\cite{paszke2019pytorch} deep learning framework and the model parameters are optimized using Adam optimizer~\cite{kingma2014adam} with momentum 0.9, beta 0.999 and weight decay set to 0. With batch size set to 32, the network is trained for 50 epochs on a single GPU. The learning rate is set to 5e-4 and is decayed by 0.1 for every 20 epochs. We do not use any pretrained weights. To have a fair comparison with baseline loss weighting methods, these hyperparameters are fixed across all the experiments.

% Human Shape Estimation Arch figure
\begin{figure*}[!htb]
    \includegraphics[scale=0.38]{figures/hsm_overview.pdf}
    {
    \captionsetup{justification=centering}
    \caption{U-Net for human shape and pose estimation} \label{fig:hsm_arch}
    }
\end{figure*}

\subsection{Pixel-wise Depth Estimation and Semantic Segmentation} \label{sec:cs_impl}
We use the training and testing split prescribed by CityScapes dataset~\cite{cordts2016cityscapes}. We closely follow the setup described in~\cite{liu2018endtoend}, which uses 7-class version of semantic labels and paired inverse depth labels, all images and labels are resized to $[128\times256]$ (see~\cite{liu2018endtoend}). We only use flip augmentation, where the image and paired labels are flipped accordingly for all the experiments. Multi-task HRNetV2 architecture is shown in Figure \ref{fig:cs_arch}. Specifically, we use HRNetV2-W48 configuration described in~\cite{sun2019highresolution} as backbone. We do not use any pretrained weights. Model parameters are optimized using Adam optimizer~\cite{kingma2014adam} with momentum 0.9, beta 0.999 and weight decay set to 0. With batch size set to 8, the network is trained for 200 epochs on a single GPU. The learning rate is set to 1e-3 and is decayed by 0.1 for every 60 epochs. To have a fair comparison with baseline loss weighting methods, these hyperparameters are fixed across all the experiments. 

% CS Arch figure
\begin{figure*}[!htb]
    \includegraphics[scale=0.38]{figures/cityscapes_overview_figure_hrnet.pdf}
     {
     \captionsetup{justification=centering}
     \caption{High resolution network \cite{sun2019highresolution} (HRNetV2-W48) for pixel-wise depth estimation and semantic segmentation} \label{fig:cs_arch}
     }
\end{figure*}


==> sub_sections/sup_training_under_noise.tex <==
\section{Learning with Noisy Annotations}

In this section we present results for controlled corruption scenario described in Section 4.6. All hyperparameters pertaining to model parameters discussed in Sections \ref{sec:hsm_impl} and \ref{sec:cs_impl} are retained as is. In SURREAL, comparison with baseline loss weighting methods when segmentation, pose and shape labels are corrupted, is presented in Tables \ref{tab:hsm_corruption_exps_segm} and \ref{tab:hsm_corruption_exps_pose}. For all the experiments in Tables \ref{tab:hsm_corruption_exps_segm} and \ref{tab:hsm_corruption_exps_pose}, learning rate for instance-level task parameters was set to 2.0. For DWA~\cite{liu2018endtoend}, temperatures 0.5 and 1.8 worked best for experiments with 20\% and 40\% corrupt segmentation labels respectively. Temperatures of 1.0 and 0.5 worked best for experiments with 20\% and 40\% corrupt pose and shape labels respectively. For various levels of corruption, our method outperforms baselines methods across all metrics.

% Noisy SURREAL results
\begin{table}[!htb]
\captionsetup{font=small}
\noindent
\begin{floatrow}
\begin{adjustbox}{width=8.2cm}
\begin{tabular}{ccccc} 
\toprule 
Method & \% Corrupt & Surface Errors & MPJPE & Pixel Accuracy \\
\midrule
Eq. Weight & & 75.69 $\pm$ 0.08 & 65.62 $\pm$ 0.09 & 97.78 $\pm$ 0.011 \\
MTU~\cite{kendall2017multitask} & & 77.15 $\pm$ 0.52 & 67.22 $\pm$ 0.54 & 97.69 $\pm$ 0.013\\
DWA~\cite{liu2018endtoend} & 20\% & 72.56 $\pm$ 0.53 & 62.50 $\pm$ 0.54 & 97.51 $\pm$ 0.094  \\
GLS~\cite{chennupati2019multinet} & & 76.60 $\pm$ 1.59 & 66.51 $\pm$ 1.43 & 97.67 $\pm$ 0.026 \\
ILT Params (Ours) & & \textbf{64.06 $\pm$ 0.45} & \textbf{54.76 $\pm$ 0.48} & \textbf{98.18 $\pm$ 0.005} \\ 
\midrule
% Best Dwa temp: 0.5

Eq. Weight & & 77.38 $\pm$ 0.71 & 67.19 $\pm$ 0.75 & 97.59 $\pm$ 0.014 \\
MTU~\cite{kendall2017multitask} & & 77.44 $\pm$ 0.39 & 67.37 $\pm$ 0.27 & 97.50 $\pm$ 0.033\\
DWA~\cite{liu2018endtoend} & 40\% & 74.02 $\pm$ 0.09 & 63.90 $\pm$ 0.08 & 97.04 $\pm$ 0.301 \\
GLS~\cite{chennupati2019multinet} & & 77.99 $\pm$ 0.93 & 67.66 $\pm$ 0.78 & 97.49 $\pm$ 0.009 \\
ILT Params (Ours) & & \textbf{65.06 $\pm$ 0.12} & \textbf{55.62 $\pm$ 0.12} & \textbf{98.07 $\pm$ 0.009} \\ 
\bottomrule
% Best dwa temp: 1.8

\end{tabular}
\end{adjustbox}
{
  \scriptsize{\caption{Comparison with baseline loss weighting methods on SURREAL test dataset for various levels of corrupt segmentation labels. Results for various loss weighting methods are from our re-implementation of the respective methods} \label{tab:hsm_corruption_exps_segm}}
}
\end{floatrow}
\end{table}

\begin{table}[!htb]
\captionsetup{font=small}
\noindent
\begin{floatrow}
\begin{adjustbox}{width=8.3cm}
\begin{tabular}{ccccc} 
\toprule 
Method & \% Corrupt & Surface Errors & MPJPE & Pixel Accuracy \\
\midrule
Eq. Weight & & 113.03 $\pm$ 3.18 & 97.67 $\pm$ 2.96 & 97.89 $\pm$ 0.009 \\
MTU~\cite{kendall2017multitask} & & 93.69 $\pm$ 2.61 & 78.90 $\pm$ 1.98 & 98.16 $\pm$ 0.003\\
DWA~\cite{liu2018endtoend} & 20\% & 110.47 $\pm$ 11.71 & 94.69 $\pm$ 10.26 & 98.07 $\pm$ 0.021 \\
GLS~\cite{chennupati2019multinet} &  & 94.68 $\pm$ 2.68 & 79.55 $\pm$ 1.96 & 98.17 $\pm$ 0.003 \\
ILT Params (Ours) & & \textbf{64.23 $\pm$ 0.81} & \textbf{55.06 $\pm$ 0.92} & \textbf{98.26 $\pm$ 0.001} \\ 
\midrule
% Best dwa temp: 1.0

Eq. Weight & & 193.91 $\pm$ 8.72 & 172.025 $\pm$ 8.24 & 97.83 $\pm$ 0.007 \\
MTU~\cite{kendall2017multitask} & & 164.80 $\pm$ 16.32 & 140.80 $\pm$ 14.21 & 98.15 $\pm$ 0.006 \\
DWA~\cite{liu2018endtoend} & 40\% & 203.87 $\pm$ 1.62 & 180.01 $\pm$ 1.44 & 98.01 $\pm$ 0.017 \\
GLS~\cite{chennupati2019multinet} & & 195.14 $\pm$ 11.47 & 168.65 $\pm$ 10.64 & 98.17 $\pm$ 0.005 \\
ILT Params (Ours) & & \textbf{66.19 $\pm$ 0.28} & \textbf{56.82 $\pm$ 0.27} & \textbf{98.27 $\pm$ 0.006} \\ 
\bottomrule
% Best dwa temp: 0.5

\end{tabular}
\end{adjustbox}
{
  \scriptsize{\caption{Comparison with baseline loss weighting methods on SURREAL test dataset for various levels of corrupt pose and shape labels. Results for various loss weighting methods are from our re-implementation of the respective methods} \label{tab:hsm_corruption_exps_pose}}
}
\end{floatrow}
\end{table}

In CityScapes, comparison with baseline loss weighting methods when segmentation and depth labels are corrupted, is presented in Tables \ref{tab:cs_corruption_exps_depth} and \ref{tab:cs_corruption_exps_segm}. For instance-level task parameters, learning rate of 0.6 and 0.4 were set for experiments with 20\% and 40\% corrupt depth labels respectively. Learning rate of 3.0 was used for all experiments with corrupt segmentation labels. For DWA~\cite{liu2018endtoend}, temperature of 2.0 worked best for all the experiments.

% Noisy Cityscapes Results
\begin{table}[!htb]
\captionsetup{font=small}
\noindent
\begin{floatrow}
\begin{adjustbox}{width=8.2cm}
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}[-3pt]{Method} & \% & \multicolumn{2}{c}{Segmentation} & \multirow{2}{*}[5.3pt]{Depth} \\ 
\cmidrule{3-5} & Corrupt & mIoU & Pix Acc & Abs Err \\ 
\midrule
Eq. Weight & & 63.14 $\pm$ 0.04 & 94.21 $\pm$ 0.14 & 0.0163 $\pm$ 0.0048 & \\
MTU~\cite{kendall2017multitask} & & 62.39 $\pm$ 0.06 & 93.95 $\pm$ 0.11 & 0.0211 $\pm$ 0.0101 & \\
DWA~\cite{liu2018endtoend} & 20\% & 63.19 $\pm$ 0.63 & 94.09 $\pm$ 0.45 & 0.0347 $\pm$ 0.0296 &  \\
GLS~\cite{chennupati2019multinet} & & 61.72 $\pm$ 0.71 & 93.89 $\pm$ 0.25 & 0.0134 $\pm$ 0.0016 & \\
ILT Params (Ours) & & \textbf{63.37 $\pm$ 0.11} &  \textbf{94.36 $\pm$ 0.08} &  \textbf{0.0128 $\pm$ 0.0008} & \\
\midrule
% Best learning rate is 0.6

Eq. Weight & & 62.77 $\pm$ 0.17 & 94.15 $\pm$ 0.14 & 0.0266 $\pm$ 0.0026  & \\
MTU~\cite{kendall2017multitask} & & 62.36 $\pm$ 0.22 & 93.96 $\pm$ 0.07 & 0.0287 $\pm$ 0.0023 & \\
DWA~\cite{liu2018endtoend} & 40\% & 62.11 $\pm$ 0.80 & 93.65 $\pm$ 0.45 & 0.0374 $\pm$ 0.0044&  \\
GLS~\cite{chennupati2019multinet} & & 61.61 $\pm$ 0.27 & 93.67 $\pm$ 0.22 & 0.0328 $\pm$ 0.0022 & \\
ILT Params (Ours) & & \textbf{63.46 $\pm$ 0.03} & \textbf{94.28 $\pm$ 0.11} & \textbf{0.0223 $\pm$ 0.0004} & \\
% \midrule
% % Best learning rate is 0.4 

\bottomrule
\end{tabular}
\end{adjustbox}
 {
  \scriptsize{\caption{Comparison with baseline loss weighting methods on CityScapes validation dataset for various levels of corrupt depth labels. Results for various loss weighting methods are from our re-implementation of the respective methods} \label{tab:cs_corruption_exps_depth}}
}
\end{floatrow}
\end{table}

\begin{table}[!htb]
\captionsetup{font=small}
\noindent
\begin{floatrow}
\begin{adjustbox}{width=8.2cm}
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}[-3pt]{Method} & \% & \multicolumn{2}{c}{Segmentation} & \multirow{2}{*}[5.3pt]{Depth} \\
\cmidrule{3-5} & Corrupt & mIoU & Pix Acc & Abs Err \\ 
\midrule

Eq. Weight & & 51.43 $\pm$ 2.32 & 88.55 $\pm$ 3.76 & 0.1209 $\pm$ 0.1460 & \\
MTU~\cite{kendall2017multitask} & & 53.56 $\pm$ 0.53 & 91.35 $\pm$ 0.52 & 0.0152 $\pm$ 0.0020 & \\
DWA~\cite{liu2018endtoend} & 20\% & 53.41 $\pm$ 0.58 & 91.42 $\pm$ 0.43 & 0.0150 $\pm$ 0.0013&  \\
GLS~\cite{chennupati2019multinet} & & 52.56 $\pm$ 0.48 & 90.31 $\pm$ 0.32 & 0.0705 $\pm$ 0.0723 & \\
ILT Params (Ours) & & \textbf{56.08 $\pm$ 0.53} & \textbf{93.50 $\pm$ 0.27} & \textbf{0.0113 $\pm$ 0.0001} & \\
\midrule
% Best learning rate is 3.0

Eq. Weight & & 42.19 $\pm$ 0.66 & 78.99 $\pm$ 1.36 & 0.0193 $\pm$ 0.0050 & \\
MTU~\cite{kendall2017multitask} & & 47.04 $\pm$ 1.94 &  85.62 $\pm$ 2.01 & 0.0185 $\pm$ 0.0057 & \\
DWA~\cite{liu2018endtoend} & 40\% & 41.55 $\pm$ 2.02 & 78.30 $\pm$ 3.56 & 0.1945 $\pm$ 0.2525 &  \\
GLS~\cite{chennupati2019multinet} & &46.95 $\pm$ 0.73 & 85.56 $\pm$ 1.13 & 0.0182 $\pm$ 0.0025 &  \\
ILT Params (Ours) & & \textbf{47.53 $\pm$ 0.87} & \textbf{86.87 $\pm$ 0.82} & \textbf{0.0123 $\pm$ 0.0005} & \\
% Best learning rate is 3.0

\bottomrule
\end{tabular}
\end{adjustbox}
{
  \scriptsize{\caption{Comparison with baseline loss weighting methods on CityScapes validation dataset for various levels of corrupt segmentation labels. Results for various loss weighting methods are from our re-implementation of the respective methods} \label{tab:cs_corruption_exps_segm}}
}
\end{floatrow}
\end{table}
